Study of the Hall effect in two different strongly correlated fermion systems

We investigate the Hall effect in two different theoretical models of strongly correlated systems: a system made of weakly coupled Luttinger liquids, in the presence of umklapp scattering, and the 2D triangular lattice, with nearest-neighbor hopping and a local Hubbard interaction. In the first model we use a memory function approach to compute the Hall coefficient as a function of temperature and frequency in the presence of umklapp scattering. We find a power-law correction to the free-fermion value (band value), with an exponent depending on the Luttinger parameter $K_{\rho}$. At sufficiently high temperature or frequency the Hall coefficient approaches the band value. We discuss the applications to Hall experiments made in quasi 1D organic compounds. In the second model, the complete temperature and doping dependencies of the high-frequency Hall coefficient $\RH$ are evaluated analytically and numerically for small, intermediate, and strong interactions using various approximation schemes. We find that $\RH$ follows the semiclassical $1/qn^*$ law near T=0, but exhibits a striking $T$-linear behavior with an interaction- and doping-dependent slope at high temperature. We compare our results with Hall measurements performed in cobaltates.

==> Latex/Classes/urlbst <==
#! /usr/bin/env perl
#
# Usage: ./urlbst.pl [--eprint] [--doi]
#    [--nohyperlinks] [--inlinelinks] [--hypertex] [--hyperref]
#    [input-file [output-file]]
# If either input-file or output-file is omitted, they are replaced by
# stdin or stdout respectively.
#
# See http://purl.org/nxg/dist/urlbst for documentation
#
# $Id: urlbst.in,v 1.8 2007/03/26 17:21:56 norman Exp $

$version = '0.6';
($progname = $0) =~ s/.*\///;
$mymarker = "% $progname";
$mymarkerend = "% ...$progname to here";
$myurl = 'http://purl.org/nxg/dist/urlbst';


$infile = '-';
$outfile = '-';

$addeprints = 0;     # if true (nonzero) we add support for eprints
$eprintprefix = 'arXiv:';	# make these settable with --eprint? syntax?
$eprinturl = 'http://arxiv.org/abs/';

$adddoiresolver = '0';
$doiprefix = 'doi:';
$doiurl = 'http://dx.doi.org/';

$makehref = 0;
$availablestring = "Available from: ";
$inlinelinks = 0;

$Usage = "$progname [--eprint] [--doi]\n    [--nohyperlinks] [--inlinelinks] [--hypertex] [--hyperref]\n    [--help] [input-file [output-file]]";

while ($#ARGV >= 0) {
    if ($ARGV[0] eq '--eprint') {
	$addeprints = 1;
    } elsif ($ARGV[0] eq '--doi') {
        $adddoiresolver = 1;
    } elsif ($ARGV[0] eq '--nohyperlinks') {
        $makehref = 0;
    } elsif ($ARGV[0] eq '--hypertex') {
	$makehref = 1;
    } elsif ($ARGV[0] eq '--hyperref') {
	$makehref = 2;
    } elsif ($ARGV[0] eq '--inlinelinks') {
        $inlinelinks = 1;
    } elsif ($ARGV[0] eq '--help') {
        print <<EOD;
urlbst version $version
    Usage: $Usage
      --eprint:       include support for `eprint' fields
      --doi:          include support for `doi' field
      --nohyperlinks  do not include active links anywhere
      --inlinelinks   add hyperlinks to entry titles
      --hypertex:     include HyperTeX-style hyperlink support
      --hyperref:     include {hyperref}-style hyperlink support
                      (generally better)
      --help:         print this help
    Input and output files may be given as `-' (default) to indicate stdin/out
EOD
        exit(0);
    } elsif ($ARGV[0] =~ /^-/) {
        die "Unrecognised option $ARGV[0]: Usage: $Usage\n";
    } elsif ($infile eq '-') {
	$infile = $ARGV[0];
    } elsif ($outfile eq '-') {
	$outfile = $ARGV[0];
    } else {
	die "Usage: $Usage\n";
    }
    shift(@ARGV);
}

if ($inlinelinks && $makehref == 0) {
    print <<'EOD';
Warning: --inlinelinks and --nohyperlinks were both specified (possibly
    implicitly).  That combination makes no sense, so I'll ignore
    --nohyperlinks and use --hyperref instead
EOD
    $makehref = 2;
}

$exitstatus = 0;		# success status

open (IN, "<$infile") || die "Can't open $infile to read";
open (OUT, ">$outfile") || die "Can't open $outfile to write";

# We have to make certain assumptions about the source files, in order
# to patch them at the correct places.  Specifically, we assume that
#
#   - there's a function init.state.consts
#
#   - ...and an output.nonnull which does the actual outputting, which
#         has the `usual' interface.
#
#   - we can replace
#           fin.entry
#       by
#           new.block
#           output.url    % the function which formats and displays any URL
#           fin.entry
#
#   - there is a function which handles the `article' entry type (this
#         will always be true)
#
#   - there is a function output.bibitem which is called at the
#         beginning of each entry type
#   - ...and one called fin.entry which is called at the end
#
# If the functions format.date, format.title or new.block are not defined (the
# former is not in apalike, for example, and the last is not in the
# AMS styles), then replacements are included in the output.
#
# All these assumptions are true of the standard files and, since most
# style files derive from them more or less directly, are true of most (?)
# other style files, too.
#
# There's some rather ugly Perl down here.  The parsing for
# brace-matching could probably do with being rewritten in places, to
# make it less ugly, and more robust.

print OUT "%%% Modification of BibTeX style file ", ($infile eq '-' ? '<stdin>' : $infile), "\n";
print OUT "%%% ... by $progname, version $version (marked with \"$mymarker\")\n%%% See <$myurl>\n";
print OUT "%%% Added webpage entry type, and url and lastchecked fields.\n";
print OUT "%%% Added eprint support.\n"   if ($addeprints);
print OUT "%%% Added DOI support.\n"      if ($adddoiresolver);
print OUT "%%% Added HyperTeX support.\n" if ($makehref == 1);
print OUT "%%% Added hyperref support.\n" if ($makehref == 2);
print OUT "%%% Original headers follow...\n\n";

$found{initconsts} = 0;
$found{outputnonnull} = 0;
$found{article} = 0;
$found{outputbibitem} = 0;
$found{finentry} = 0;
$found{formatdate} = 0;
$found{formattitle} = 0;
$found{newblock} = 0;

while (<IN>) {
    /^ *%/ && do {
        # Pass commented lines unchanged
        print OUT;
        next;
    };
    
    /^ *ENTRY/ && do {
	# Work through the list of entry types, finding what ones are there.
	# If we find a URL entry there already, object, since these edits
	# will mess things up.
	$line = $_;
	until ($line =~ /\{\s*(\w*)/) {
	    $line .= <IN>;
	}
	$bracematchtotal = 0;	# reset
	bracematcher($line);
	$line =~ /\{\s*(\w*)/;
	$found{'entry'.$1} = 1;
	print OUT $line;
	$line = <IN>;
	until (bracematcher($line) == 0) {
	    # XXX deal with multiple entries on one line
	    ($line =~ /^\s*(\w*)/) && ($found{'entry'.$1} = 1);
	    print OUT $line;
	    $line = <IN>;
	}
	if (defined($found{entryurl})) {
	    print STDERR "$progname: style file $infile already has URL entry!\n";
	    # print out the rest of the file, and give up
            print OUT $line;
	    while (<IN>) {
		print OUT;
	    }
	    $exitstatus = 1;
	    last;
	} else {
            print OUT "    eprint $mymarker\n    doi $mymarker\n    url $mymarker\n    lastchecked $mymarker\n";
	}
	print OUT $line;
	next;
    };

    /^ *FUNCTION *\{init\.state\.consts\}/ && do {
        # In the init.state.consts function, add an extra set of
        # constants at the beginning.  Also use this as the marker for
        # the place to add the init strings function.
        print OUT <<EOD;
STRINGS { urlintro eprinturl eprintprefix doiprefix doiurl openinlinelink closeinlinelink } $mymarker...
INTEGERS { hrefform inlinelinks makeinlinelink addeprints adddoiresolver }
% Following constants may be adjusted by hand, if desired
FUNCTION {init.urlbst.variables}
{
  "$availablestring" 'urlintro := % prefix before URL
  "$eprinturl" 'eprinturl := % prefix to make URL from eprint ref
  "$eprintprefix" 'eprintprefix := % text prefix printed before eprint ref
  "$doiurl" 'doiurl := % prefix to make URL from DOI
  "$doiprefix" 'doiprefix :=      % text prefix printed before DOI ref
  #$addeprints 'addeprints :=         % 0=no eprints; 1=include eprints
  #$adddoiresolver 'adddoiresolver :=     % 0=no DOI resolver; 1=include it
  #$makehref 'hrefform :=           % 0=no crossrefs; 1=hypertex xrefs; 2=hyperref refs
  #$inlinelinks 'inlinelinks :=        % 0=URLs explicit; 1=URLs attached to titles
  % the following are internal state variables, not config constants
  #0 'makeinlinelink :=     % state variable managed by setup.inlinelink
  "" 'openinlinelink :=     % ditto
  "" 'closeinlinelink :=    % ditto
}
INTEGERS { 
  bracket.state
  outside.brackets
  open.brackets
  within.brackets
  close.brackets
}
$mymarkerend
EOD
	$line = $_;
	until ($line =~ /\{.*\}.*\{/s) {
	    $line .= <IN>;
	}
	$line =~ s/(\{.*?\}.*?\{)/$1 #0 'outside.brackets := $mymarker
  #1 'open.brackets :=
  #2 'within.brackets :=
  #3 'close.brackets :=

 /s;
	print OUT $line;
	$found{initconsts} = 1;
	next;
    };

    /^ *EXECUTE *\{init\.state\.consts\}/ && do {
        print OUT "EXECUTE {init.urlbst.variables}\n";
        print OUT;
        next;
    };

    /^ *FUNCTION *\{new.block\}/ && do {
        $found{newblock} = 1;
    };

    /^ *FUNCTION *{output\.nonnull}/ && do {
	print OUT "$mymarker\n";
	print OUT "FUNCTION {output.nonnull.original}\n";
        copy_block();
	print_output_functions();
	$found{outputnonnull} = 1;
	next;
    };

    /FUNCTION *\{fin.entry\}/ && do {
        # Rename fin.entry to fin.entry.original (wrapped below)
        s/fin.entry/fin.entry.original/;
        $found{finentry} = 1;
        print OUT;
        next;
    };

    /^ *FUNCTION *{format\.date}/ && do {
	$found{formatdate} = 1;
	print OUT;
	next;
    };

    /^ *FUNCTION *{format\.title}/ && do {
        # record that we found this
	$found{formattitle} = 1;
        print OUT;
	next;
    };

    /^ *format\.b?title/ && do {
        # interpolate a call to setup.inlinelink
        print OUT "  title empty\$ 'skip\$ 'setup\.inlinelink if\$ $mymarker\n";
        print OUT;
        next;
    };

    /^ *FUNCTION *\{article\}/ && do {

	print_missing_functions();
	print_webpage_def();

	print OUT;
	$found{article} = 1;
	next;
    };

    /FUNCTION *\{output.bibitem\}/ && do {
        # Rename output.bibitem to output.bibitem.original (wrapped below)
        s/{output.bibitem\}/\{output.bibitem.original\}/;
 	$found{outputbibitem} = 1;
        print OUT;
        next;
    };

    print OUT;
};

if ($exitstatus == 0) {
    # Skip this if we've already reported an error -- it'll only be confusing
    foreach $k (keys %found) {
        if ($found{$k} == 0) {
            print STDERR "$progname: $infile: failed to find feature $k\n";
        }
    }
}

close (IN);
close (OUT);

exit $exitstatus;;






sub print_output_functions {
    print OUT "$mymarker...\n";

    print OUT <<'EOD';
% The following three functions are for handling inlinelink.  They wrap
% a block of text which is potentially output with write$ by multiple
% other functions, so we don't know the content a priori.
% They communicate between each other using the variables makeinlinelink
% (which is true if a link should be made), and closeinlinelink (which holds
% the string which should close any current link.  They can be called
% at any time, but start.inlinelink will be a no-op unless something has
% previously set makeinlinelink true, and the two ...end.inlinelink functions
% will only do their stuff if start.inlinelink has previously set
% closeinlinelink to be non-empty.
FUNCTION {setup.inlinelink}
{ makeinlinelink
    { hrefform #1 = % hypertex
        { "\special {html:<a href=" quote$ * url * quote$ * "> }{" * 'openinlinelink :=
          "\special {html:</a>}" 'closeinlinelink :=
          }
        { hrefform #2 = % hyperref
            { "\href{" url * "}{" * 'openinlinelink :=
              "}" 'closeinlinelink :=
              }
            'skip$
          if$ % hrefform #2 =
        }
      if$ % hrefform #1 =
      #0 'makeinlinelink :=
    }
    'skip$
 if$ % makeinlinelink
}
FUNCTION {add.inlinelink}
{ openinlinelink empty$
    'skip$
    { openinlinelink swap$ * closeinlinelink *
      "" 'openinlinelink :=
      }
  if$
}
EOD

    # new.block is defined elsewhere

    print OUT <<'EOD';
FUNCTION {output.nonnull}
{ % Save the thing we've been asked to output
  's :=
  % If the bracket-state is close.brackets, then add a close-bracket to
  % what is currently at the top of the stack, and set bracket.state
  % to outside.brackets
  bracket.state close.brackets =
    { "]" *
      outside.brackets 'bracket.state :=
    }
    'skip$
  if$
  bracket.state outside.brackets =
    { % We're outside all brackets -- this is the normal situation.
      % Write out what's currently at the top of the stack, using the
      % original output.nonnull function.
      s
      add.inlinelink
      output.nonnull.original % invoke the original output.nonnull
    }
    { % Still in brackets.  Add open-bracket or (continuation) comma, add the
      % new text (in s) to the top of the stack, and move to the close-brackets
      % state, ready for next time (unless inbrackets resets it).  If we come
      % into this branch, then output.state is carefully undisturbed.
      bracket.state open.brackets =
        { " [" * }
        { ", " * } % bracket.state will be within.brackets
      if$ 
      s * 
      close.brackets 'bracket.state :=
    }
  if$
}

% Call this function just before adding something which should be presented in 
% brackets.  bracket.state is handled specially within output.nonnull.
FUNCTION {inbrackets}
{ bracket.state close.brackets =
    { within.brackets 'bracket.state := } % reset the state: not open nor closed
    { open.brackets 'bracket.state := }
  if$
}

FUNCTION {format.lastchecked}
{ lastchecked empty$
    { "" }
    { inbrackets "cited " lastchecked * }
  if$
}
EOD
    print OUT "$mymarkerend\n";
}

sub print_webpage_def {
    print OUT "$mymarker...\n";

    # Some of the functions below call new.block, so we need a dummy
    # version, in the case where the style being edited doesn't supply
    # that function.
    if (! $found{newblock}) {
        print OUT "FUNCTION {new.block} % dummy new.block function\n{\n  % empty\n}\n\n";
        $found{newblock} = 1;
    }

    print OUT <<'EOD';
% Functions for making hypertext links.
% In all cases, the stack has (link-text href-url)
%
% make 'null' specials
FUNCTION {make.href.null}
{
  pop$
}
% make hypertex specials
FUNCTION {make.href.hypertex}
{ 
  "\special {html:<a href=" quote$ *
  swap$ * quote$ * "> }" * swap$ *
  "\special {html:</a>}" *
}
% make hyperref specials
FUNCTION {make.href.hyperref}
{ 
  "\href {" swap$ * "} {\path{" * swap$ * "}}" *
}
FUNCTION {make.href}
{ hrefform #2 =
    'make.href.hyperref      % hrefform = 2
    { hrefform #1 =
        'make.href.hypertex  % hrefform = 1
        'make.href.null      % hrefform = 0 (or anything else)
      if$
    }
  if$
}

% If inlinelinks is true, then format.url should be a no-op, since it's
% (a) redundant, and (b) could end up as a link-within-a-link.
FUNCTION {format.url}
{ inlinelinks #1 = url empty$ or
   { "" }
   { hrefform #1 =
       { % special case -- add HyperTeX specials
         urlintro "\url{" url * "}" * url make.href.hypertex * }
       { urlintro "\url{" * url * "}" * }
     if$
   }
  if$
}

FUNCTION {format.eprint}
{ eprint empty$
    { "" }
    { eprintprefix eprint * eprinturl eprint * make.href }
  if$
}

FUNCTION {format.doi}
{ doi empty$
    { "" }
    { doiprefix doi * doiurl doi * make.href }
  if$
}

% Output a URL.  We can't use the more normal idiom (something like
% `format.url output'), because the `inbrackets' within
% format.lastchecked applies to everything between calls to `output',
% so that `format.url format.lastchecked * output' ends up with both
% the URL and the lastchecked in brackets.
FUNCTION {output.url}
{ url empty$
    'skip$ 
    { new.block 
      format.url output
      format.lastchecked output 
    }
  if$
}

FUNCTION {output.web.refs}
{
  new.block
  output.url
  addeprints eprint empty$ not and
    { format.eprint output.nonnull }
    'skip$
  if$
  adddoiresolver doi empty$ not and
    { format.doi output.nonnull }
    'skip$
  if$
}

% Wrapper for output.bibitem.original.
% If the URL field is not empty, set makeinlinelink to be true,
% so that an inline link will be started at the next opportunity
FUNCTION {output.bibitem}
{ outside.brackets 'bracket.state :=
  output.bibitem.original
  inlinelinks url empty$ not and
    { #1 'makeinlinelink := }
    { #0 'makeinlinelink := }
  if$
}

% Wrapper for fin.entry.original
FUNCTION {fin.entry}
{ output.web.refs  % urlbst
  makeinlinelink       % ooops, it appears we didn't have a title for inlinelink
    { setup.inlinelink % add some artificial link text here, as a fallback
      "[link]" output.nonnull }
    'skip$
  if$
  bracket.state close.brackets = % urlbst
    { "]" * }
    'skip$
  if$
  fin.entry.original
}

% Webpage entry type.
% Title and url fields required;
% author, note, year, month, and lastchecked fields optional
% See references 
%   ISO 690-2 http://www.nlc-bnc.ca/iso/tc46sc9/standard/690-2e.htm
%   http://www.classroom.net/classroom/CitingNetResources.html
%   http://neal.ctstateu.edu/history/cite.html
%   http://www.cas.usf.edu/english/walker/mla.html
% for citation formats for web pages.
FUNCTION {webpage}
{ output.bibitem
  author empty$
    { editor empty$
        'skip$  % author and editor both optional
        { format.editors output.nonnull }
      if$
    }
    { editor empty$
        { format.authors output.nonnull }
        { "can't use both author and editor fields in " cite$ * warning$ }
      if$
    }
  if$
  new.block
  title empty$ 'skip$ 'setup.inlinelink if$
  format.title "title" output.check
  inbrackets "online" output
  new.block
  year empty$
    'skip$
    { format.date "year" output.check }
  if$
  % We don't need to output the URL details ('lastchecked' and 'url'),
  % because fin.entry does that for us, using output.web.refs.  The only
  % reason we would want to put them here is if we were to decide that
  % they should go in front of the rather miscellaneous information in 'note'.
  new.block
  note output
  fin.entry
}
EOD

    print OUT "$mymarkerend\n\n\n";
}


sub print_missing_functions {
    # We've got to the bit of the file which handles the entry
    # types, so write out the webpage entry handler.  This uses
    # the format.date function, which which many but not all
    # bst files have (for example, apalike doesn't).  So
    # check that we either have found this function already, or
    # add it.
    if (! $found{formatdate}) {
	if ($found{entrymonth}) {
	    print OUT <<'EOD';
FUNCTION {format.date}
{ year empty$
    { month empty$
	{ "" }
	{ "there's a month but no year in " cite$ * warning$
	  month
	}
      if$
    }
    { month empty$
	'year
	{ month " " * year * }
      if$
    }
  if$
}
EOD
	} else {
	    print OUT <<'EOD';
FUNCTION {format.date}
{ year empty$
    'skip$
    { %write$
      "(" year * ")" *
    }
  if$
}
EOD
  	}
	$found{formatdate} = 1;
    }

    # If the style file didn't supply a format.title function, then supply
    # one here (the {webpage} function requires it).
    if (! $found{formattitle}) {
	print OUT <<'EOD';
FUNCTION {format.title}
{ title empty$
    { "" }
    { title "t" change.case$ }
  if$
}
EOD
    $found{formattitle} = 1;
    }
}

# Utility function: Keep track of open and close braces in the string argument.
# Keep state in $bracematchtotal, return the current value.
sub bracematcher {
    my $s = shift;
    $s =~ s/[^\{\}]//g;
    #print "s=$s\n";
    foreach my $c (split (//, $s)) {
	$bracematchtotal += ($c eq '{' ? 1 : -1);
    }
    return $bracematchtotal;
}

# Utility function: use bracematcher to copy the complete block which starts
# on or after the current line.
sub copy_block {
    $bracematchtotal = 0;
    # copy any leading lines which don't have braces (presumably comments)
    while (defined ($line = <IN>) && ($line !~ /{/)) {
        print OUT $line;
    }
    while (defined ($line) && bracematcher($line) > 0) {
        print OUT $line;
        $line = <IN>;
    }
    print OUT "$line\n";	# print out terminating \} (assumed
    				# alone on the line)
}


==> X.tex <==
\relax 
\@setckpt{Frontmatter/acknowledgement}{
\setcounter{page}{96}
\setcounter{equation}{4}
\setcounter{enumi}{0}
\setcounter{enumii}{0}
\setcounter{enumiii}{0}
\setcounter{enumiv}{0}
\setcounter{footnote}{0}
\setcounter{mpfootnote}{0}
\setcounter{part}{0}
\setcounter{chapter}{2}
\setcounter{section}{3}
\setcounter{subsection}{0}
\setcounter{subsubsection}{0}
\setcounter{paragraph}{0}
\setcounter{subparagraph}{0}
\setcounter{figure}{1}
\setcounter{table}{0}
\setcounter{parentequation}{4}
}


==> glossary.tex <==
% this file is called up by thesis.tex
% content in this file will be fed into the main document

% Glossary entries are defined with the command \nomenclature{1}{2}
% 1 = Entry name, e.g. abbreviation; 2 = Explanation
% You can place all explanations in this separate file or declare them in the middle of the text. Either way they will be collected in the glossary.

% required to print nomenclature name to page header
\markboth{\MakeUppercase{\nomname}}{\MakeUppercase{\nomname}}


% ----------------------- contents from here ------------------------

% chemicals
\nomenclature{DAPI}{4',6-diamidino-2-phenylindole; a fluorescent stain that binds strongly to DNA and serves to marks the nucleus in fluorescence microscopy} 
\nomenclature{DEPC}{diethyl-pyro-carbonate; used to remove RNA-degrading enzymes (RNAases) from water and laboratory utensils}
\nomenclature{DMSO}{dimethyl sulfoxide; organic solvent, readily passes through skin, cryoprotectant in cell culture}
\nomenclature{EDTA}{Ethylene-diamine-tetraacetic acid; a chelating (two-pronged) molecule used to sequester most divalent (or trivalent) metal ions, such as calcium (Ca$^{2+}$) and magnesium (Mg$^{2+}$), copper (Cu$^{2+}$), or iron (Fe$^{2+}$ / Fe$^{3+}$)}




